QA-Align: Representing Cross-Text Content Overlap by Aligning Question-Answer Propositions

Multi-text applications, such as multi-document summarization, are typically required to model redundancies across related texts. Current methods confronting consolidation struggle to fuse overlapping information. In order to explicitly represent content overlap, we propose to align predicate-argument relations across texts, providing a potential scaffold for information consolidation. We go beyond clustering coreferring mentions, and instead model overlap with respect to redundancy at a propositional level, rather than merely detecting shared referents. Our setting exploits QA-SRL, utilizing question-answer pairs to capture predicate-argument relations, facilitating laymen annotation of cross-text alignments. We employ crowd-workers for constructing a dataset of QA-based alignments, and present a baseline QA alignment model trained over our dataset. Analyses show that our new task is semantically challenging, capturing content overlap beyond lexical similarity and complements cross-document coreference with proposition-level links, offering potential use for downstream tasks.

==> tables/align_ex.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{ll}
\multicolumn{2}{l}{Sentence A: [A  man  and  three  women ]AL1 were \textbf{arrested}  [outside  the  white house ]AL2 after the president’s speech.} \\ \hline
\multicolumn{2}{l}{Sentence B: A journalist was interviewing the [4 people ]AL1 that were \textbf{charged}  [outside the president’s house ]AL2.} \\ \hline
Role & QA \\ \hline
Pred: Arrested A1: \textit{arrestee? criminal} & Who was arrested somewhere? --- A man and three women \\
Pred: Charged A1: \textit{assigned} & Who was charged with something? --- 4 people \\
\multirow{2}{*}{\textit{LOC: location}} & Where was someone arrested? \\
 & Where was someone charged? --- outside the president's house
\end{tabular}%
}
\caption{An example of two alignments aligning the patient (A1) (arestee) and the Location role. Below is an example of the aligned predicate-argument relations modeled using QASRL}
\label{tab:align_qasrl_role_ex}
\end{table*}

==> tables/align_qa_ex_2.tex <==
\begin{table*}[h]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lll}
\multicolumn{3}{l}{Sentence A: Wade \textbf{purchased} Cunningham's home in San Diego for over  \$1.6M and a few months later sold it for a \$700,000 loss ...} \\
\multicolumn{3}{l}{Sentence B: Federal agencies are investigating Rep. Randall "Duke" Cunningham for \textbf{selling} his house to a military contractor, Mitchell Wade ...} \\ \hline
\multicolumn{1}{c}{\textbf{Aligned QAs from Sentence A}} &  & \multicolumn{1}{c}{\textbf{Aligned QAs from Sentence B}} \\
Who \textbf{purchased} something? --- Wade & ---- Alignment 1 ---- & Who did someone \textbf{sell} something to? --- Mitchell Wade \\
What did someone \textbf{purchase}? --- Cunningham 's home & ---- Alignment 2 ---- & What did someone \textbf{sell} to someone? --- his house
\end{tabular}%
}
\caption{An example of two alignments expressing the same propositions captured by QASRL question-answers.}
\label{tab:align_qasrl_ex}
\end{table*}

==> tables/align_qasrl_ex.tex <==
\begin{table*}[h]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{ll}
\multicolumn{2}{l}{Sentence A: An earthquake measuring 4 . 6 rattled Sonoma and Lake counties early Thursday ...} \\
\multicolumn{2}{l}{Sentence B: The temblor struck about 26 miles north of Santa Rosa in the Geysers area.}        \\ \hline
\textbf{Aligned QAs from Sentence A}                              & \textbf{Aligned QAs from Sentence B}          \\
What rattled something? - An earthquake measuring 4 . 6           & Who struck somewhere? - The temblor           \\
What did something rattle? - Sonoma and Lake counties &
  \begin{tabular}[c]{@{}l@{}}Where did someone strike? - \\ about 26 miles north of Santa Rosa in the Geysers area\end{tabular}
\end{tabular}%
}
\caption{An example of two alignments, represented by QASRL question-answers.}
\label{tab:align_qasrl_old}
\end{table*}

==> tables/fusion_dataset.tex <==
\begin{table*}[hbt!]
\centering
\begin{tabular}{ l|p{2cm}|p{2cm}|p{2cm}|p{2cm} }
Data Source & \# instances & Avg Cluster size & Avg Rouge Label & Avg Rouge Input\\ \hline
Thadani & 1644 & 2.76 & 0.42&-\\
This work - pyramid data & 6722 & 2.85 & 0.30&- \\
This work - doc data & 1459 & 3.57 & 0.16&-\\
Poc lebanoff & 1599 & 2 & 0.25&-\\

\end{tabular}
\caption{A comparison of multiple variations of fusion datasets. Rouge scores are macro averages of rouge 1, 2, and L. Rouge label refers to scores of fusion labels and each of their sentence input, while Rouge Input refers to sentence pairs in a shared fusion input. Cluster size represents number of sentences in a fusion input instance.}
\label{tab:fusion_data}
\end{table*}
%Delta pyramid & 5078 & 2.88 & 0.27\\ Removed this one, probably don't need

==> tables/many_align_ex.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}

\begin{table*}[t!]
\textwidth
\begin{tabular}{ll}
\multicolumn{1}{l|}{Sentence A} & \begin{tabular}[c]{@{}l@{}}... he will resign Friday after [his wife\textsubscript{A0}] was [\textbf{hospitalized}\textsubscript{pred}]\\ Thursday night ''due to an ongoing ailment,'' CNN reports.\end{tabular}\\ \cline{2-2} 
\multicolumn{1}{l|}{Sentence B} & \begin{tabular}[c]{@{}l@{}} ... Last night, my [wife\textsubscript{A0}] was [\textbf{admitted}\textsubscript{pred}] to 
 [the hospital\textsubscript{A1}]\\ 
 in Washington, D.C., due to an ongoing ailment.''\end{tabular}\\
\multicolumn{2}{l}{}\\
\multicolumn{1}{l|}{Alignment} & A: Who was \textbf{hospitalized}? - his wife\\ \cline{2-2} 
\multicolumn{1}{l|}{} & B: Who was \textbf{admitted} somewhere? - wife\\
\multicolumn{1}{l|}{} & B: Where was someone \textbf{admitted} to? - the hospital
\end{tabular}%
\caption{An example of paired sentences from MultiNews, and a corresponding single alignment. We treat this an alignment of the Agent relation (or "person hospitalized") as a 1-to-many alignment, showcasing a light-verb construction phenomena, where a single verb 'hospitalized' is semantically equivalent to 'admitted to hospital'. \dan{is the text too depressing? not sure this is they right way to show a many2many} }
\label{tab:many_align_ex}
\end{table*}

==> tables/qasrl_ex.tex <==
\begin{table*}[hbt!]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{ll}
\multicolumn{2}{l}{Several reservations have successfully established casinos that \textbf{provide} income to alleviate extreme poverty.} \\ \hline
Role & QA \\ \hline
A0: provider, agent & What \textbf{provides} something? - casinos \\
A1: thing provided, theme & What does something \textbf{provide}? - income \\
Adj, why? & Why does something \textbf{provide} something? - to alleviate extreme poverty
\end{tabular}%
}
\caption{Example of predicate-argument relations modeled using QASRL}
\label{tab:qasrl_ex}
\end{table*}
